Topological turbulence in spin-orbit-coupled driven-dissipative quantum fluids of light generates high angular momentum states

We demonstrate the formation of a high angular momentum turbulent state in an exciton-polariton quantum fluid with TE-TM Spin-Orbit Coupling (SOC). The transfer of particles from quasi-resonantly cw pumped \spl component to \sm component is accompanied with the generation of a turbulent gas of quantum vortices by inhomogeneities. We show that this system is unstable with respect to the formation of bogolons at a finite wave vector, controlled by the laser detuning. In a finite-size cavity, the domains with this wave vector form a ring-like structure along the border of a cavity, with a gas of mostly same-sign vortices in the center. The total angular momentum is imposed by the sign of TE-TM SOC, the wave vector of instability, and the cavity size. This effect can be detected experimentally via local dispersion measurements or by interference. The proposed configuration thus allows simultaneous experimental studies of quantum turbulence and high-angular momentum states in continuously-pumped exciton-polariton condensates.

==> stuff.tex <==
%In 2D, this process is expected to be isotropic is k-space, unless the system symmetry is broken. This symmetry breaking is provided by the flow created by the topological quantum turbulence.
%There are two types of excitations in 2D quantum fluids: quantum vortices, and density waves called bogolons which are generated through virtual parametric processes. Above some threshold these virtual processes become real ones and become amplified
%In this work we show that TE-TM coupling can be used to conduct the turbulence studies in exciton-polaritons. The problem of phase pinning under the quasi-resonant pumping and the problem of finite polariton lifetime was already solved by employment of the so-called pump/support scheme \cite{pigeon2017sustained,soln2019vortexstreet,claude2020taming,lerario2020parallel} using the bistability. However, the vortices/vortex chains/solitons were stationary in time, which is not appropriate for the studies of turbulence requiring a gas of the free-moving quantum vortices. The use of a spinor polariton quantum fluids brings an extra degree of freedom and the above mentioned problem becomes solved. We propose to use the CW pump of the \spl component and to detect in the opposite \sm component. At the same time, the ``automatic'' stirring and creation of free vortices (due to angular momentum transfer by TE-TM SOC) will take place in the \sm component, which is an essential step to obtain the desired turbulent regime. As a result we generate a gas of nearly free quantum vortices in the \sm component under quasi-resonant pumping of the \spl component.

The behavior of the system can be explained as follows. At the first stage the high density in \spl component is formed and the transfer to \an{the} \sm component starts. One observes the nearly linear regime in the \sm component with the massive vortices generation similarly to OSHE and the complex phase patterns defined by the interference of multiple waves. At the same time, the predicted instability is manifested as domains at a definite wave vector. The sign of $\Delta N$ is defined by the angular momentum transfer direction imposed by TE-TM splitting. 





During the transitional regime, the high-density domains are created due to instability at $k_0$. They expand and undergo the specular reflection at the border of a cavity. The domains then continue following the border with the direction defined by the global rotational flow due to disequilibrium in the number of left and right vortices stemming from the sign of TE-TM splitting. The flow is supersonic due to relatively low density in the \sm component. Finally, the domains form a ring-like structure following the borders, while the free vortex gas remains at in the bulk of the cavity pillar (Fig. \ref{fig_phase_and_time_depend}b)).

%The system of exciton-polaritons with effective magnetic fields demonstrates rich behavior with transfer of energy, particles, momentum, angular momentum between the components, appearance of topological phenomena. At the same time, the non-linearity, the essential attribute of polariton quantum fluids at high densities, leads to existence of topological defects like solitons and quantum vortices, which are well visible in real experiments. As shown previously, operation with the laser power within or close to bistability loop allows solving the phase locking problem, which is essential for development of the complex-phase topological defects \cite{pigeon2017sustained,soln2019vortexstreet}. Still, the vortices/vortex chains/solitons are shaped by the stable in time WF and do not move that is an obstacle for studies of turbulence being a gas of the free-moving quantum vortices.

%The quantum fluids can also manifest the quantum turbulence regime with sufficient stochasticity and randomness of flows and kinetic energy stored in the rotational motion defined by the ensembles of quantum vortices.
%\textbf{Also to cite: TE-TM Savenko \cite{kovalev2017paramagnetic} and Vortices Yulin and Anton \cite{yulin2020spinning}}
